On the Dynamics of Solid, Liquid and Digital Gold Futures

This paper examines the determinants of the volatility of futures prices and basis for three commodities: gold, oil and bitcoin -- often dubbed solid, liquid and digital gold -- by using contract-by-contract analysis which has been previously applied to crude oil futures volatility investigations. By extracting the spot and futures daily prices as well as the maturity, trading volume and open interest data for the three assets from 18th December 2017 to 30th November 2021, we find a positive and significant role for trading volume and a possible negative influence of open interest, when significant, in shaping the volatility in all three assets, supporting earlier findings in the context of oil futures. Additionally, we find maturity has a relatively positive significance for bitcoin and oil futures price volatility. Furthermore, our analysis demonstrates that maturity affects the basis of bitcoin and gold positively -- confirming the general theory that the basis converges to zero as maturity nears for bitcoin and gold -- while oil is affected in both directions.

==> sections/5-future_work.tex <==
\section{Future Work}

\textcolor{red}{Other commodities such as oil.}

Features of the CME Bitcoin futures contract, combined with the relative nascency of the financial product, resulted in a small sample size. Therefore, it is likely that evidence of market inefficiency would not have been detected even if it did exist. Thus future work can apply the methodology proposed to larger data sets when they become available, or to try with other Bitcoin future markets data. For example, Kraken offers several futures contract pairs, including BTC/USD, ETH/USD, LTCUSD,	BCH/USD, XRP/USD and XRP/BTC. Also, OKEx and BitMEX, although they are unregulated marketplaces, each have average daily volumes exceeding \$1 billion, making them the two largest bitcoin futures exchanges available today. Testing with data from these markets would ensure robustness of the empirical results.

Additionally, larger data sets would enable us introduce autoregressive moving average (ARMA) model\footnote{ARMA models provide a description of a weak stationary stochastic process in terms of two processes: Autoregression (AR($p$)) model and Moving average (MA($q$)) model. The model is usually referred to as ARMA($p,q$) model where $p$ is the number of AR terms and $q$ is the number of MA terms. The AR part denotes regressing the variable on its own lagged (i.e., past) series values. The MA part models the error term as a linear combination of residual terms of various times in the past.}, as tested in \cite{CANARELLA1986575,Otto2011}. The ARMA approach is one of the promising ways to empirically test the speculative efficiency hypothesis with overlapping data sets, which avoid reducing the sample size and loss of information. We omitted this method as from the econometric point of view, the rule of thumb is that at least 50, but ideally more than 100 observations, should be estimated for ARMA models \cite{Box1975} and our samples doesn't meet this criteria. For the CME Bitcoin futures overlapping price to be analyzed with ARMA, we need to wait for enough data to be accumulated, unless new types of commodities emerges.


%We find that 1-month Bitcoin futures prices are not unbiased estimators of future Bitcoin spot prices. This suggests that the market for 1-month Bitcoin futures is inefficient, implying the possibility for excess returns. On the other hand, for 2-week and 1-week futures prices, we are unable to reject the null hypothesis that futures prices are unbiased predictors of future Bitcoin spot prices. On top of this, we found the Bitcoin futures price becomes a more accurate indicator of the spot price as the futures contract becomes shorter. This leads to the conclusion that the current 1-month Bitcoin futures price is not an unbiased estimator of the future Bitcoin spot price, and hence making room for excess returns, but that the market becomes more efficient as the contract length shortens.

%Future work includes the application of the methodology proposed to larger data sets or to test different Bitcoin futures markets data. This is because the features of the CME Bitcoin futures contract prohibited us from obtaining high frequency data enough to test with daily observations. Testing with data from these markets would guarantee robustness of the empirical results. Additionally, larger data sets would enable us introduce an autoregressive moving average (ARMA) model, as tested in \cite{CANARELLA1986575,Otto2011}. Utilizing the ARMA approach would make it possible for us to empirically test the speculative efficiency hypothesis with overlapping data, which avoid reducing the sample size.


==> sections/annex.tex <==
\section{Appendix}
This annex gives additional tables, regression results and figures to complement the paper. See main text for further discussion.

\subsection{CBDC projects status}

Below shows the part of the updated project score of global CBDC development efforts, relating to \cite{BIS_Auer2020} (as of December 2020)\footnote{The dataset includes all projects announced as of 1 December 2020. For more information, see \url{https://www.bis.org/publ/work880.htm}.}. Note that only the countries with index of 3 (live CBDC) and 2 (pilot) as of December 2020 are listed here.

\begin{table}[htbp]
%\caption{Table captions should be placed above the tables.}\label{tab:variables}
\begin{tabular}{l|c c c c}
\toprule
\textbf{Country} &~~ \textbf{Overall*} &~~ \textbf{Overall (Aug 20)} &~~ \textbf{Retail*} &~~ \textbf{Wholesale*}\\ \hline
Bahamas &~~ 3 &~~ 2 &~~ 3 &~~ 0\\
Canada &~~	3 &~~ 2 &~~ 1 &~~ 2\\
Switzerland	&~~ 3 &~~ 1	&~~ 1 &~~ 2\\
Euro area (ECB)	&~~ 3	&~~ 2 &~~ 1 &~~ 2\\
France &~~ 3 &~~ 2	&~~ 1	&~~ 2\\
Japan &~~ 3 &~~ 2 &~~ 1 &~~ 2\\
South Africa &~~ 3 &~~ 1 &~~ 1 &~~ 2\\
United Arab Emirates~~ &~~ 2 &~~	2 &~~	0 &~~ 2\\
Australia &~~	2 &~~	1 &~~	1 &~~	1\\
China &~~	2 &~~	2 &~~	2 &~~	0\\
Ecuador &~~	2 &~~	2 &~~	2 &~~	0\\
Eastern Caribbean &~~	2 &~~	2 &~~	2 &~~ 0\\
United Kingdom &~~ 2 &~~ 2 &~~	1 &~~	1\\
Hong Kong &~~	2 &~~	2 &~~	0 &~~	2\\
Indonesia &~~	2 &~~	1 &~~	1 &~~	1\\
India &~~	2 &~~	0 &~~	1 &~~	1\\
South Korea &~~	2 &~~	2 &~~	2 &~~	0\\
Saudi Arabia &~~	2 &~~	2 &~~	0 &~~	2\\
Sweden &~~	2 &~~	2 &~~	2 &~~	0\\
Singapore &~~	2 &~~	2 &~~	0 &~~	2\\
Swaziland &~~	2 &~~	1 &~~	1 &~~	1\\
Thailand &~~	2 &~~	2 &~~	0 &~~	2\\
Ukraine &~~	2 &~~	2 &~~	2 &~~	0\\
Uruguay &~~	2 &~~	2&~~	2 &~~	0\\
\bottomrule
\addlinespace[1ex]
\multicolumn{3}{l}{*As of December 2020.}
\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{8mm}
\subsection{Table of observed variables}\label{sec:variables}
The following table lists the observed variables included in our analysis.
\begin{table*}[h]
%\caption{Table captions should be placed above the tables.}\label{tab:variables}
\begin{tabular}{l l c}
\toprule
\textbf{Variable} & ~~\textbf{Description} & \textbf{Source}\\ \hline
\addlinespace[1ex]
\textbf{Digital infrastructure}\\
Mobile subscriptions & ~~Mobile cellular subscriptions (per 100 people) & WB\\
Secure Internet & ~~Secure Internet servers (per 1 million people)  & WB\\
Fixed broadband & ~~Fixed broadband subscriptions (per 100 people) & WB\\
indiv. Internet use & ~~Individuals using the Internet (\% of population) & WB\\
\addlinespace[2ex]
%%%
\multicolumn{2}{l}{\textbf{Development and financial inclusion}}\\
Account ownership  &
\begin{tabular}{l}
~Account ownership at a financial institution or with a\\~mobile-money-service provider (\% of population ages 15+) 
\end{tabular}& WB\\
FD index & ~~Financial development index & IMF\cite{Svirydzenka2016}\\
GDP per capita & ~~GDP divided by midyear population (USD)  & WB\\
\addlinespace[2ex]
%%%
\multicolumn{2}{l}{\textbf{Institutional characteristics}}\\
Government effectiveness & ~~Quality of public services, policy implementation etc. & IMF\\
Regulatory quality & ~~Ability to formulate and implement sound policies etc. & IMF\\
Voice and accountability & ~~Extent of citizens' participation and freedom expression & IMF\\

\addlinespace[2ex]
\multicolumn{2}{l}{\textbf{Innovation environment}}\\
Access to electricity & ~~Access to electricity (\% of population) & WB\\

\addlinespace[2ex]
\multicolumn{2}{l}{\textbf{Demographic characteristics}}\\
\% of people over 65
 & ~~Total population 65 years of age or older & WB \\
 
\addlinespace[2ex]
\multicolumn{2}{l}{\textbf{Cross-border transactions}}\\
Trade (\% of GDP) & ~~Sum of exports and imports (\% of GDP) & WB \\

%\addlinespace[2ex]
%\multicolumn{2}{l}{\textbf{Public interest in CBDCs}}\\
%Search interest & ~~Google/Baidu & BIS \\

\bottomrule
\addlinespace[1ex]
\multicolumn{3}{l}{Source: World Bank, IMF, BIS (online annex of \cite{BIS_Auer2020}).} % Added
\end{tabular}
\end{table*}

%Digital infrastructure data comes from International Telecommunication Union.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\subsection{Top 10 features for the random forest classifier with aggregated data}
\label{ssec:top-features}
Table~\ref{tab:important-features_2008} and \ref{tab:important-features_2012} give the 10 most important independent variables for the random forest classifier with aggregated data (data averaged over the period 2014–19, subject to data availability), with August 2020 and December 2020 CBDCPI data as an objective variable, respectively.
\begin{table}[h]
    \caption{Most important features for the random forest classifier (Aug 2020)}
    \label{tab:important-features_2008}
    \setlength{\tabcolsep}{10pt}
    \centering
    \begin{tabular}{l c}
        \toprule
        \bf Feature & \bf Importance\\
        \midrule
        Financial Development Index & 0.165\\
        GDP per capita & 0.098\\
        Voice and accountability & 0.095\\
        Broadband subscriptions (per 100 people) & 0.093\\
        Government effectiveness & 0.087\\
        \% of people over 65 & 0.082\\
        Individuals using the Internet (\% of population) & 0.080\\
        Trade (\% of GDP) & 0.078\\
        Secure Internet servers (per 1 million people) & 0.072\\
        Regulatory quality & 0.068\\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[h]
    \caption{Most important features for the random forest classifier (Dec 2020)}
    \label{tab:important-features_2012}
    \setlength{\tabcolsep}{10pt}
    \centering
    \begin{tabular}{l c}
        \toprule
        \bf Feature & \bf Importance\\
        \midrule
        \% of people over 65 & 0.134\\
        Financial Development Index & 0.109\\
        Mobile cellular subscriptions (per 100 people) & 0.101\\
        GDP per capita & 0.090\\
        Voice and accountability & 0.089\\  Secure Internet servers (per 1 million people) & 0.086\\   
        Individuals using the Internet (\% of population) & 0.080\\
        Government effectiveness & 0.080\\
        Broadband subscriptions (per 100 people) & 0.076\\
        Trade (\% of GDP) & 0.067\\        
        \bottomrule
    \end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\subsection{Top 10 features for the random forest classifier with full data}
\label{ssec:top-features_full}
Table~\ref{tab:important-features_full2008} and \ref{tab:important-features_full2012} show the 10 most important index for the random forest classifier with full data, with August 2020 and December 2020 CBDCPI data as an objective variable, respectively.
\begin{table}[h]
    \caption{Most important features for the random forest classifier (Aug 2020)}
    \label{tab:important-features_full2008}
    \setlength{\tabcolsep}{10pt}
    \centering
    \begin{tabular}{l c}
        \toprule
        \bf Feature & \bf Importance\\
        \midrule
        Financial Development Index & 0.052\\
        Government effectiveness [YR2019] & 0.033\\
        Government effectiveness [YR2018] & 0.020\\
        Broadband subscriptions (per 100 people) [YR2017] & 0.020\\
        Individuals using the Internet (\% of population) [YR2012]& 0.020\\
        Individuals using the Internet (\% of population) [YR2015]& 0.020\\
        GDP per capita [YR2016] & 0.018\\
        Government effectiveness [YR2015] & 0.016\\
        Mobile cellular subscriptions (per 100 people) [YR2016]& 0.015\\
        \% of people over 65 [YR1990]& 0.014\\
        \bottomrule
    \end{tabular}
\end{table}


\begin{table}[h]
    \caption{Most important features for the random forest classifier (Dec 2020)}
    \label{tab:important-features_full2012}
    \setlength{\tabcolsep}{10pt}
    \centering
    \begin{tabular}{l c}
        \toprule
        \bf Feature & \bf Importance\\
        \midrule
        Financial Development Index & 0.037\\
        \% of people over 65 [YR1990] & 0.035\\
        Mobile cellular subscriptions (per 100 people) [YR2019] & 0.025\\
        \% of people over 65 [YR2018] & 0.023\\
        \% of people over 65 [YR2017] & 0.021\\
        \% of people over 65 [YR2000] & 0.020\\
        Government effectiveness [YR2017] & 0.020\\
        \% of people over 65 [YR2015] & 0.020\\
        \% of people over 65 [YR2013] & 0.019\\
        Mobile cellular subscriptions (per 100 people) [YR2015] & 0.018\\       
        \bottomrule
    \end{tabular}
\end{table}


